A Verified Information-Flow Architecture

SAFE is a clean-slate design for a highly secure computer system, with pervasive mechanisms for tracking and limiting information flows. At the lowest level, the SAFE hardware supports fine-grained programmable tags, with efficient and flexible propagation and combination of tags as instructions are executed. The operating system virtualizes these generic facilities to present an information-flow abstract machine that allows user programs to label sensitive data with rich confidentiality policies. We present a formal, machine-checked model of the key hardware and software mechanisms used to dynamically control information flow in SAFE and an end-to-end proof of noninterference for this model. We use a refinement proof methodology to propagate the noninterference property of the abstract machine down to the concrete machine level. We use an intermediate layer in the refinement chain that factors out the details of the information-flow control policy and devise a code generator for compiling such information-flow policies into low-level monitor code. Finally, we verify the correctness of this generator using a dedicated Hoare logic that abstracts from low-level machine instructions into a reusable set of verified structured code generators.

==> Makefile <==
ifeq ($(USER),demange)
  OTT = "/Users/demange/ott_distro_0.21.2/bin/ott"
else
  OTT = "$(shell which ott || echo \"$(HOME)\"/bin/ott)"
endif

PDFLATEX = pdflatex -halt-on-error -synctex=-1

all: temp/main.tex temp/defns.tex
	$(MAKE) once
	$(PDFLATEX) $<
	$(PDFLATEX) $<
	-sed -i -e 's/temp\/main.tex/main.tex/g' main.synctex
	cp main.pdf temp/temp.pdf

once:  temp/main.tex temp/defns.tex 
	-$(PDFLATEX) $<
	-bibtex main
	-sed -i -e 's/temp\/main.tex/main.tex/g' main.synctex
	cp main.pdf temp/temp.pdf

# You can get pulp here: https://github.com/dmwit/pulp
PULP = "$(shell which pulp || echo \"$(HOME)\"~/.cabal/bin/pulp)"

pulp: temp/main.tex temp/defns.tex
	rm -f main.log
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-bibtex main
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-$(PDFLATEX) -interaction nonstopmode $< &> /dev/null
	-sed -i -e 's/temp\/main.tex/main.tex/g' main.synctex
	-$(PULP) main.log

clean:
	@ rm -rf temp *.aux *.log main.pdf 
	@ rm -rf *~ *.log main.pdf *.out *.bbl *.blg main.synctex.gz

temp/defns.tex: defns.ott Makefile
	if [ ! -d "temp" ]; then mkdir temp; fi
	${OTT} -tex_wrap false -i defns.ott -o temp/defns.tex

temp/main.tex: main.tex temp/defns.tex
	if [ ! -d "temp" ]; then mkdir temp; fi
	${OTT} -i defns.ott -tex_wrap false -tex_filter $< $@

DATE = $(shell date --i)

release-techreport:
	rm -dfr techrep techrep-$(DATE).zip
	mkdir techrep
	cp Makefile techrep
	cp main.tex techrep
	cp *.bst *.sty *.bib *.ott report.cls techrep
	cp main.log.pulp techrep
	echo "\draftfalse\techreptrue" > techrep/texdirectives.tex
	cp local.bib ../../safe.bib techrep
	sed -i 's/\.\.\/\.\.\///g' techrep/main.tex
	make -C techrep pulp
	mv techrep/temp/main.tex techrep/main.tex
	rm techrep/main.synctex
	rm techrep/*.bib # they explicitly ask for it
	mv techrep/main.pdf techrep-$(DATE).pdf
	cd techrep; zip -r ../techrep-$(DATE).zip *

.PHONY : all once clean


==> texdirectives.tex <==
\draftfalse\techreptrue

